lpcde: Estimation and Inference for Local Polynomial Conditional Density Estimators

This paper discusses the R package lpcde, which stands for local polynomial conditional density estimation. It implements the kernel-based local polynomial smoothing methods introduced in Cattaneo, Chandak, Jansson, Ma (2024) for statistical estimation and inference of conditional distributions, densities, and derivatives thereof. The package offers mean square error optimal bandwidth selection and associated point estimators, as well as uncertainty quantification based on robust bias correction both pointwise (e.g., confidence intervals) and uniformly (e.g., confidence bands) over evaluation points. The methods implemented are boundary adaptive whenever the data is compactly supported. The package also implements regularized conditional density estimation methods, ensuring the resulting density estimate is non-negative and integrates to one. We contrast the functionalities of lpcde with existing open-source packages for conditional density estimation, and showcase its main features using simulated and real datasets. An abbreviated version of this article is published in Cattaneo, Chandak, Jansson, Ma (2025 JOSS).

==> _markdown_CCJM_JOSS/bf3781a0285075f0247f571c608e7188.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererSectionBegin
\markdownRendererHeadingOne{Summary}\markdownRendererInterblockSeparator
{}Conditional cumulative distribution functions (CDFs), probability density functions (PDFs), and derivatives thereof, are important parameters of interest in statistics, econometrics, and other data science disciplines. The package 'lpcde' implements a new method for estimation of and inference of conditional CDFs, PDFs, and derivatives thereof, by employing the kernel-based local polynomial smoothing approach introduced in \markdownRendererCodeSpan{@CCJM:2024}.\markdownRendererInterblockSeparator
{}Building on the theoretical and methodological work reported in \markdownRendererCodeSpan{@CCJM:2024}, the package 'lpcde' offers data-driven (pointwise and uniform) estimation and inference methods for conditional CDFs, PDFs, and derivatives thereof, which are automatically valid at interior, and boundary points on the support of both the variable of interest and the conditioning variables. For point estimation, the package offers mean squared error optimal bandwidth selection and associated point estimators. For inference, the package offers valid confidence intervals and confidence bands based on robust bias-correction techniques \markdownRendererCodeSpan{@Calonico-Cattaneo-Farrell\markdownRendererUnderscore{}2018\markdownRendererUnderscore{}JASA,Calonico-Cattaneo-Farrell\markdownRendererUnderscore{}2022\markdownRendererUnderscore{}Bernoulli}. Finally, these statistical procedures can be easily used for visualization and graphical presentation of smooth empirical CDFs, PDFs, and derivative thereof with custom 'ggplot'\markdownRendererCodeSpan{[@ggplot2]} commands built for the package.\markdownRendererInterblockSeparator
{}This package is currently the only open-source estimator across multiple programming languages that provides adaptive conditional density estimation with robust bias-correction and pointwise confidence interval and uniform confidence band construction, providing users with tools to better understand the reliability of their analysis. Additional information including a detailed tutorial on using the package and replication files can be found on the \markdownRendererLink{GitHub repository}{https://nppackages.github.io/lpcde/}{https://nppackages.github.io/lpcde/}{} or through the \markdownRendererLink{CRAN repository}{https://cran.r-project.org/web/packages/lpcde/index.html}{https://cran.r-project.org/web/packages/lpcde/index.html}{}.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingOne{Statement of need}\markdownRendererInterblockSeparator
{}\markdownRendererCodeSpan{@Wand-Jones\markdownRendererUnderscore{}1995\markdownRendererUnderscore{}Book}, \markdownRendererCodeSpan{@Fan-Gijbels\markdownRendererUnderscore{}1996\markdownRendererUnderscore{}Book}, \markdownRendererCodeSpan{@simonoff2012smoothing}, and \markdownRendererCodeSpan{@scott2015multivariate} give textbook introductions to kernel-based density and local polynomial estimation and inference methods. The core idea underlying the estimator implemented in 'lpcde' is to use kernel-based local polynomial smoothing methods to construct an automatically boundary adaptive estimator for CDFs, PDFs, and derivatives thereof. The estimator implemented in this package consists of two steps. The first step estimates the conditional distribution function using standard local polynomial regression methods, and the second step applies local polynomial smoothing to the (non-smooth) local polynomial conditional CDF estimate from the first step to obtain a smooth estimate of the CDF, PDF, and derivatives thereof.\markdownRendererInterblockSeparator
{}A distinct advantage of this estimation method over existing ones is that the estimator is boundary adaptive (i.e. accurate and reliable) for a possibly unknown compact support of the data. Furthermore, the estimator has a simple closed form representation, which leads to easy and fast implementation. Unlike some other boundary adaptive procedures, this estimation procedure does not require pre-processing of data, and thus avoids the challenges of hyper-parameter tuning: only one bandwidth parameter needs to be selected for implementation.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingOne{Comparing and Contrasting Existing Toolsets}\markdownRendererInterblockSeparator
{}The package 'lpcde' contributes to a rather small set of open-source software packages for estimation and inference about conditional CDF, PDF, and derivatives thereof. More specifically, we identified two 'R' packages: 'hdrcde'\markdownRendererTilde{}\markdownRendererCodeSpan{[@hdrcde]'}and 'np'\markdownRendererCodeSpan{[@np]}, and one 'Python' package: 'cde'\markdownRendererCodeSpan{[@rothfuss2019conditional]}, which provide related methodology. There are no open-source 'Stata' packages that implement conditional CDF, PDF, and derivative thereof estimation. The table summarizes some of the main differences between those packages and 'lpcde'. As is noted in the table, 'lpcde' is the only package available across multiple programming languages that provides both pointwise and uniform confidence interval construction that is asymptotically valid, in addition to producing boundary adaptive estimates, and proper conditional density estimates that are non-negative and integrate to one. These features are unique contributions of the package to the overall 'R' (and more broadly, open-source programming) toolkit.\markdownRendererInterblockSeparator
{}\markdownRendererPipe{} Package \markdownRendererPipe{} Programming language \markdownRendererPipe{} CDF/Derivative estimation \markdownRendererPipe{} Regularized density \markdownRendererPipe{} Valid at boundary \markdownRendererPipe{} Standard error \markdownRendererPipe{} Valid inference \markdownRendererPipe{} Confidence bands \markdownRendererPipe{} Bandwidth selection \markdownRendererPipe{} \markdownRendererPipe{}---\markdownRendererPipe{}---\markdownRendererPipe{}:---:\markdownRendererPipe{}---:\markdownRendererPipe{}---\markdownRendererPipe{}---\markdownRendererPipe{}---\markdownRendererPipe{}---\markdownRendererPipe{}---\markdownRendererPipe{} \markdownRendererPipe{} hdrcde \markdownRendererPipe{} R \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [x] \markdownRendererPipe{} \markdownRendererPipe{} np \markdownRendererPipe{} R \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [x]\markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [x] \markdownRendererPipe{} \markdownRendererPipe{} cde \markdownRendererPipe{} Python \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [x] \markdownRendererPipe{} \markdownRendererPipe{} lpcde \markdownRendererPipe{} R \markdownRendererPipe{} [x] \markdownRendererPipe{} [x] \markdownRendererPipe{} [x] \markdownRendererPipe{} [x] \markdownRendererPipe{} [x] \markdownRendererPipe{} [x] \markdownRendererPipe{} [x] \markdownRendererPipe{}
\markdownRendererSectionEnd \markdownRendererDocumentEnd

==> _markdown_CCJM_JOSS/efb1bd669917f8202cec83df9bd7ca08.md.tex <==
\markdownRendererDocumentBegin
\markdownRendererSectionBegin
\markdownRendererHeadingOne{Summary}\markdownRendererInterblockSeparator
{}Conditional cumulative distribution functions (CDFs), probability density functions (PDFs), and derivatives thereof, are important parameters of interest in statistics, econometrics, and other data science disciplines. The package 'lpcde' implements a new method for estimation of and inference of conditional CDFs, PDFs, and derivatives thereof, by employing the kernel-based local polynomial smoothing approach introduced in \markdownRendererCodeSpan{@CCJM:2024}.\markdownRendererInterblockSeparator
{}Building on the theoretical and methodological work reported in \markdownRendererCodeSpan{@CCJM:2024}, the package 'lpcde' offers data-driven (pointwise and uniform) estimation and inference methods for conditional CDFs, PDFs, and derivatives thereof, which are automatically valid at interior, and boundary points on the support of both the variable of interest and the conditioning variables. For point estimation, the package offers mean squared error optimal bandwidth selection and associated point estimators. For inference, the package offers valid confidence intervals and confidence bands based on robust bias-correction techniques \markdownRendererCodeSpan{@Calonico-Cattaneo-Farrell\markdownRendererUnderscore{}2018\markdownRendererUnderscore{}JASA,Calonico-Cattaneo-Farrell\markdownRendererUnderscore{}2022\markdownRendererUnderscore{}Bernoulli}. Finally, these statistical procedures can be easily used for visualization and graphical presentation of smooth empirical CDFs, PDFs, and derivative thereof with custom 'ggplot'\markdownRendererCodeSpan{[@ggplot2]} commands built for the package.\markdownRendererInterblockSeparator
{}This package is currently the only open-source estimator across multiple programming languages that provides adaptive conditional density estimation with robust bias-correction and pointwise confidence interval and uniform confidence band construction, providing users with tools to better understand the reliability of their analysis. Additional information including a detailed tutorial on using the package and replication files can be found on the \markdownRendererLink{GitHub repository}{https://nppackages.github.io/lpcde/}{https://nppackages.github.io/lpcde/}{} or through the \markdownRendererLink{CRAN repository}{https://cran.r-project.org/web/packages/lpcde/index.html}{https://cran.r-project.org/web/packages/lpcde/index.html}{}.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingOne{Statement of need}\markdownRendererInterblockSeparator
{}\markdownRendererCodeSpan{@Wand-Jones\markdownRendererUnderscore{}1995\markdownRendererUnderscore{}Book}, \markdownRendererCodeSpan{@Fan-Gijbels\markdownRendererUnderscore{}1996\markdownRendererUnderscore{}Book}, \markdownRendererCodeSpan{@simonoff2012smoothing}, and \markdownRendererCodeSpan{@scott2015multivariate} give textbook introductions to kernel-based density and local polynomial estimation and inference methods. The core idea underlying the estimator implemented in 'lpcde' is to use kernel-based local polynomial smoothing methods to construct an automatically boundary adaptive estimator for CDFs, PDFs, and derivatives thereof. The estimator implemented in this package consists of two steps. The first step estimates the conditional distribution function using standard local polynomial regression methods, and the second step applies local polynomial smoothing to the (non-smooth) local polynomial conditional CDF estimate from the first step to obtain a smooth estimate of the CDF, PDF, and derivatives thereof.\markdownRendererInterblockSeparator
{}A distinct advantage of this estimation method over existing ones is that the estimator is boundary adaptive (i.e. accurate and reliable) for a possibly unknown compact support of the data. Furthermore, the estimator has a simple closed form representation, which leads to easy and fast implementation. Unlike some other boundary adaptive procedures, this estimation procedure does not require pre-processing of data, and thus avoids the challenges of hyper-parameter tuning: only one bandwidth parameter needs to be selected for implementation.\markdownRendererInterblockSeparator
{}
\markdownRendererSectionEnd \markdownRendererSectionBegin
\markdownRendererHeadingOne{Comparing and Contrasting Existing Toolsets}\markdownRendererInterblockSeparator
{}The package 'lpcde' contributes to a rather small set of open-source software packages for estimation and inference about conditional CDF, PDF, and derivatives thereof. More specifically, we identified two 'R' packages: 'hdrcde'\markdownRendererTilde{}\markdownRendererCodeSpan{[@hdrcde]}and 'np'\markdownRendererCodeSpan{[@np]}, and one 'Python' package: 'cde'\markdownRendererCodeSpan{[@rothfuss2019conditional]}, which provide related methodology. There are no open-source 'Stata' packages that implement conditional CDF, PDF, and derivative thereof estimation. The table summarizes some of the main differences between those packages and 'lpcde'. As is noted in the table, 'lpcde' is the only package available across multiple programming languages that provides both pointwise and uniform confidence interval construction that is asymptotically valid, in addition to producing boundary adaptive estimates, and proper conditional density estimates that are non-negative and integrate to one. These features are unique contributions of the package to the overall 'R' (and more broadly, open-source programming) toolkit.\markdownRendererInterblockSeparator
{}\markdownRendererPipe{} Package \markdownRendererPipe{} Programming language \markdownRendererPipe{} CDF/Derivative estimation \markdownRendererPipe{} Regularized density \markdownRendererPipe{} Valid at boundary \markdownRendererPipe{} Standard error \markdownRendererPipe{} Valid inference \markdownRendererPipe{} Confidence bands \markdownRendererPipe{} Bandwidth selection \markdownRendererPipe{} \markdownRendererPipe{}---\markdownRendererPipe{}---\markdownRendererPipe{}:---:\markdownRendererPipe{}---:\markdownRendererPipe{}---\markdownRendererPipe{}---\markdownRendererPipe{}---\markdownRendererPipe{}---\markdownRendererPipe{}---\markdownRendererPipe{} \markdownRendererPipe{} hdrcde \markdownRendererPipe{} R \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [x] \markdownRendererPipe{} \markdownRendererPipe{} np \markdownRendererPipe{} R \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [x]\markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [x] \markdownRendererPipe{} \markdownRendererPipe{} cde \markdownRendererPipe{} Python \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [] \markdownRendererPipe{} [x] \markdownRendererPipe{} \markdownRendererPipe{} lpcde \markdownRendererPipe{} R \markdownRendererPipe{} [x] \markdownRendererPipe{} [x] \markdownRendererPipe{} [x] \markdownRendererPipe{} [x] \markdownRendererPipe{} [x] \markdownRendererPipe{} [x] \markdownRendererPipe{} [x] \markdownRendererPipe{}
\markdownRendererSectionEnd \markdownRendererDocumentEnd
